A Novel Benchmark and Dataset for Efficient 3D Gaussian Splatting with Gaussian Point Cloud Compression

Recently, immersive media and autonomous driving applications have significantly advanced through 3D Gaussian Splatting (3DGS), which offers high-fidelity rendering and computational efficiency. Despite these advantages, 3DGS as a display-oriented representation requires substantial storage due to its numerous Gaussian attributes. Current compression methods have shown promising results but typically neglect the compression of Gaussian spatial positions, creating unnecessary bitstream overhead. We conceptualize Gaussian primitives as point clouds and propose leveraging point cloud compression techniques for more effective storage. AI-based point cloud compression demonstrates superior performance and faster inference compared to MPEG Geometry-based Point Cloud Compression (G-PCC). However, direct application of existing models to Gaussian compression may yield suboptimal results, as Gaussian point clouds tend to exhibit globally sparse yet locally dense geometric distributions that differ from conventional point cloud characteristics. To address these challenges, we introduce GausPcgc for Gaussian point cloud geometry compression along with a specialized training dataset GausPcc-1K. Our work pioneers the integration of AI-based point cloud compression into Gaussian compression pipelines, achieving superior compression ratios. The framework complements existing Gaussian compression methods while delivering significant performance improvements. All code, data, and pre-trained models will be publicly released to facilitate further research advances in this field.

==> alg/fractal.tex <==
\begin{algorithm}
\caption{Fractal Dimension Calculation for Point Clouds}
\label{algor:fractal}
\begin{algorithmic}[1]
\Require Point cloud datasets $\{\mathcal{P}_d\}_{d=1}^D$, voxel size $\epsilon_0$
\Ensure Fractal dimension sequences $\{f_x^{(d)}\}_{d=1}^D$ for all datasets

\Function{ComputeFractalDimension}{$\mathcal{P}$, $\epsilon_0$}
    \State \textcolor{blue}{// Phase 1: Voxelization and multi-scale representation}
    \State \ensuremath{\mathcal{X} \gets \mathrm{Voxelize}(\mathcal{P}, \epsilon_0)} \Comment{Voxelize point cloud}
    \State \ensuremath{\mathcal{X}^{(0)} \gets \mathcal{X}} \Comment{Initialize finest scale representation}
    
    \State \ensuremath{l \gets 0} \Comment{Scale level counter}
    \State \ensuremath{\{N_l\} \gets [|\mathcal{X}^{(0)}|]} \Comment{Initialize voxel count sequence}
    \State \ensuremath{\{\mathcal{X}^{(l)}\}_{l=0}^L \gets [\mathcal{X}^{(0)}]} \Comment{Store multi-scale representation}
    
    \State \textcolor{blue}{// Phase 2: Iterative downsampling}
    \While{\ensuremath{|\mathcal{X}^{(l)}| > 1}} \Comment{Continue until only one voxel remains}
        \State \ensuremath{\mathcal{X}^{(l+1)} \gets \mathcal{D}(\mathcal{X}^{(l)})} \Comment{Downsample using stride-2 convolution}
        \State \ensuremath{N_{l+1} \gets |\mathcal{X}^{(l+1)}|} \Comment{Count voxels at new scale}
        \State \ensuremath{\{N_l\} \gets \{N_l\} \cup \{N_{l+1}\}} \Comment{Append to voxel count sequence}
        \State \ensuremath{\{\mathcal{X}^{(l)}\}_{l=0}^L \gets \{\mathcal{X}^{(l)}\}_{l=0}^L \cup \{\mathcal{X}^{(l+1)}\}}
        \State \ensuremath{l \gets l + 1}
    \EndWhile
    
    \State \ensuremath{L \gets l} \Comment{Total number of scales}
    
    \State \textcolor{blue}{// Phase 3: Compute fractal dimension between adjacent scales}
    \State \ensuremath{\{f_x^{(l)}\}_{l=1}^L \gets [\ ]} \Comment{Initialize fractal dimension sequence}
    
    \For{\ensuremath{l = 1} \textbf{to} \ensuremath{L}}
        \State \ensuremath{f_x^{(l)} \gets \log_2(N_{l-1}/N_l)} \Comment{Compute using Eq.~\ref{fractal dimension cal}}
        \State \ensuremath{\{f_x^{(l)}\}_{l=1}^L \gets \{f_x^{(l)}\}_{l=1}^L \cup \{f_x^{(l)}\}}
    \EndFor
    
    \State \ensuremath{\bar{D}_B \gets \frac{1}{L}\sum_{l=1}^{L}f_x^{(l)}} \Comment{Compute average fractal dimension}
    
    \State \Return \ensuremath{\{f_x^{(l)}\}_{l=1}^L, \bar{D}_B}
\EndFunction

\State \textcolor{blue}{// Phase 4: Process all datasets}
\State \ensuremath{\{f_x^{(d)}\}_{d=1}^D \gets [\ ]} \Comment{Store fractal dimensions for all datasets}
\State \ensuremath{\{\bar{D}_B^{(d)}\}_{d=1}^D \gets [\ ]} \Comment{Store average dimensions for all datasets}

\For{\ensuremath{d = 1} \textbf{to} \ensuremath{D}}
    \State \ensuremath{\{f_x^{(d)}\}_{l=1}^{L_d}, \bar{D}_B^{(d)} \gets \text{ComputeFractalDimension}(\mathcal{P}_d, \epsilon_0)}
    \State \ensuremath{\{f_x^{(d)}\}_{d=1}^D \gets \{f_x^{(d)}\}_{d=1}^D \cup \{\{f_x^{(d)}\}_{l=1}^{L_d}\}}
    \State \ensuremath{\{\bar{D}_B^{(d)}\}_{d=1}^D \gets \{\bar{D}_B^{(d)}\}_{d=1}^D \cup \{\bar{D}_B^{(d)}\}}
\EndFor

\State \textcolor{blue}{// Phase 5: Align and compare fractal dimensions across datasets}
\State \ensuremath{L_{min} \gets \min_{d=1}^D L_d} \Comment{Find minimum sequence length}

\State \textcolor{blue}{// Phase 6: Calculate dataset statistics}
\For{\ensuremath{l = 1} \textbf{to} \ensuremath{L_{min}}}
    \State \ensuremath{\bar{f}_x^{(l)} \gets \frac{1}{D}\sum_{d=1}^{D}f_x^{(d)}(l)} \Comment{Cross-dataset average at scale $l$}
    \State \ensuremath{\sigma_l \gets \sqrt{\frac{1}{D}\sum_{d=1}^{D}(f_x^{(d)}(l) - \bar{f}_x^{(l)})^2}} \Comment{Standard deviation at scale $l$}
\EndFor

\State \Return \ensuremath{\{f_x^{(d)}\}_{d=1}^D, \{\bar{D}_B^{(d)}\}_{d=1}^D, \{\bar{f}_x^{(l)}\}_{l=1}^{L_{min}}, \{\sigma_l\}_{l=1}^{L_{min}}}
\end{algorithmic}
\end{algorithm}

==> alg/local.tex <==
\begin{algorithm}
\caption{Local Density Analysis}
\label{algor:local density}
\begin{algorithmic}[1]
\Require Point cloud datasets $\{\mathcal{P}_d\}_{d=1}^D$, voxel size $\tau$, neighborhood size $k$
\Ensure Probability density functions $\{\hat{p}_d^{(l)}(n)\}_{d=1}^D$ for all datasets at each scale $l$

\Function{ProcessDataset}{$\mathcal{P}_d$, $\tau$, $k$}
    \State \textcolor{blue}{// Phase 1: Multi-scale representation construction}
    \State \ensuremath{\mathcal{X} \gets \mathrm{Voxelize}(\mathcal{P}_d, \tau)} \Comment{Voxelize using Eq.~\ref{eq:voxelize}}
    \State \ensuremath{\mathcal{X}^{(0)} \gets \mathcal{X}} \Comment{Initialize finest scale representation}
    
    \State \ensuremath{l \gets 0} \Comment{Scale level counter}
    \State \ensuremath{\{\mathcal{X}^{(l)}\} \gets [\mathcal{X}^{(0)}]} \Comment{Initialize multi-scale representation}
    
    \While{\ensuremath{|\mathcal{X}^{(l)}| > 1}} \Comment{Continue until only one voxel remains}
        \State \ensuremath{\mathcal{X}^{(l+1)} \gets \mathcal{D}(\mathcal{X}^{(l)})} \Comment{Downsample using Eq.~\ref{eq:downsample}}
        \State \ensuremath{\{\mathcal{X}^{(l)}\} \gets \{\mathcal{X}^{(l)}\} \cup \{\mathcal{X}^{(l+1)}\}}
        \State \ensuremath{l \gets l + 1}
    \EndWhile
    
    \State \ensuremath{L \gets l} \Comment{Total number of scales}
    \State \ensuremath{\{p_d^{(l)}(n)\}_{l=0}^L \gets [\ ]} \Comment{Initialize density functions for all scales}
    
    \State \textcolor{blue}{// Phase 2: Neighborhood density calculation for each scale}
    \For{\ensuremath{l = 0} \textbf{to} \ensuremath{L}}
        \State \ensuremath{\{N(v^{(l)}_i)\}_{v^{(l)}_i \in \mathcal{X}^{(l)}} \gets [\ ]} \Comment{Initialize neighborhood counts}
        
        \For{\ensuremath{\text{each voxel } v^{(l)}_i \in \mathcal{X}^{(l)}}}
            \State \ensuremath{N(v^{(l)}_i) \gets \sum_{u \in \mathcal{N}_k(v^{(l)}_i)} \mathbb{I}_{\mathcal{X}^{(l)}}(u)} \Comment{Compute using Eq.~\ref{eq:neighborhood}}
            \State \ensuremath{\{N(v^{(l)}_i)\}_{v^{(l)}_i \in \mathcal{X}^{(l)}} \gets \{N(v^{(l)}_i)\}_{v^{(l)}_i \in \mathcal{X}^{(l)}} \cup \{N(v^{(l)}_i)\}}
        \EndFor
        
        \State \textcolor{blue}{// Phase 3: Probability density function estimation}
        \State \ensuremath{\{b_j\}_{j=0}^B \gets \text{LinSpace}(0, k^3, B+1)} \Comment{Create histogram bins}
        \State \ensuremath{h^{(l)}(b_j) \gets \text{Histogram}(\{N(v^{(l)}_i)\}, \{b_j\})} \Comment{Compute using Eq.~\ref{eq:histogram}}
        \State \ensuremath{p_d^{(l)}(n) \gets h^{(l)}(b_j)} \Comment{Store normalized histogram as PDF}
        
        \State \ensuremath{\{p_d^{(l)}(n)\}_{l=0}^L \gets \{p_d^{(l)}(n)\}_{l=0}^L \cup \{p_d^{(l)}(n)\}}
    \EndFor
    
    \State \Return \ensuremath{\{p_d^{(l)}(n)\}_{l=0}^L}
\EndFunction

\State \textcolor{blue}{// Phase 4: Process all datasets}
\State \ensuremath{\{\{\hat{p}_d^{(l)}(n)\}_{l=0}^{L_d}\}_{d=1}^D \gets [\ ]} \Comment{Initialize PDFs for all datasets}

\For{\ensuremath{d = 1} \textbf{to} \ensuremath{D}}
    \State \ensuremath{\{p_d^{(l)}(n)\}_{l=0}^{L_d} \gets \text{ProcessDataset}(\mathcal{P}_d, \tau, k)}
    \State \ensuremath{\{\{\hat{p}_d^{(l)}(n)\}_{l=0}^{L_d}\}_{d=1}^D \gets \{\{\hat{p}_d^{(l)}(n)\}_{l=0}^{L_d}\}_{d=1}^D \cup \{\{p_d^{(l)}(n)\}_{l=0}^{L_d}\}}
\EndFor

\State \textcolor{blue}{// Phase 5: Distribution comparison across datasets}
\State \ensuremath{L_{min} \gets \min_{d=1}^D L_d} \Comment{Find minimum number of scales across datasets}

\For{\ensuremath{l = 0} \textbf{to} \ensuremath{L_{min}}}
    \For{\ensuremath{i = 1} \textbf{to} \ensuremath{D}}
        \For{\ensuremath{j = i+1} \textbf{to} \ensuremath{D}}
            \State \ensuremath{D_{KL}(\hat{p}_i^{(l)} \| \hat{p}_j^{(l)}) \gets \int_0^{k^3} \hat{p}_i^{(l)}(n) \log \frac{\hat{p}_i^{(l)}(n)}{\hat{p}_j^{(l)}(n)} dn} \Comment{Using Eq.~\ref{eq:kldiv}}
            \State \ensuremath{\text{Store } D_{KL}(\hat{p}_i^{(l)} \| \hat{p}_j^{(l)}) \text{ for datasets } i \text{ and } j \text{ at scale } l}
        \EndFor
    \EndFor
\EndFor

\State \Return \ensuremath{\{\{\hat{p}_d^{(l)}(n)\}_{l=0}^{L_{min}}\}_{d=1}^D \text{ and KL divergence measures}}
\end{algorithmic}
\end{algorithm}
